Semi-Supervised Deep Learning for Abnormality Classification in Retinal Images

Supervised deep learning algorithms have enabled significant performance gains in medical image classification tasks. But these methods rely on large labeled datasets that require resource-intensive expert annotation. Semi-supervised generative adversarial network (GAN) approaches offer a means to learn from limited labeled data alongside larger unlabeled datasets, but have not been applied to discern fine-scale, sparse or localized features that define medical abnormalities. To overcome these limitations, we propose a patch-based semi-supervised learning approach and evaluate performance on classification of diabetic retinopathy from funduscopic images. Our semi-supervised approach achieves high AUC with just 10-20 labeled training images, and outperforms the supervised baselines by upto 15% when less than 30% of the training dataset is labeled. Further, our method implicitly enables interpretation of the SSL predictions. As this approach enables good accuracy, resolution and interpretability with lower annotation burden, it sets the pathway for scalable applications of deep learning in clinical imaging.

==> extra.tex <==
% JMB: I think this entire paragraph can be skipped. It's quite detailed, so I've made a more concise version at the end of the previous sentence
% However, annotation of medical images is laborious, time-consuming and relies on expensive clinical expertise. Further, annotation of medical images is often compounded by two factors that increase the annotation burden. First, the annotations can be noisy due to inter-rater variability even among clinical experts \cite{Campbell2016Plus,Krause2017}. Often, this variability is addressed by acquiring multiple blinded ratings per image, particularly in clinical validation data sets used to assess final performance \cite{Gulshan2016,Krause2017}. Second, in some use cases, good performance can only be obtained with very fine pixel or ROI-level annotations [CITE]. The prohibitive nature of acquiring detailed consensus annotations from multiple clinical experts on million-scale medical image data have led researchers to rely on weights from networks that are pre-trained on general scene databases (e.g., ImageNet, CIFAR-10, etc) \cite{JiaDeng2009,Krizhevsky2014Cifar}. However, such workarounds carry the risk of neglecting critical clinical information, and do not apply to common clinical scenarios involving cross-sectional (3D) imaging or video data. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Our semi-supervised approach is based on Generative Adversarial Networks (GANs) \cite{goodfellow2014generative}. GANs are a class of deep generative neural network models that have been successful in modeling distributions over natural images \cite{Radford2015}. A typical GAN consists of a generator network $G$ and discriminator network $D$. In the course of training a GAN on a set of (unlabeled) images, the generator learns how to map a low-dimensional set of random variables $Z$ to generate images, while the discriminator learns how to differentiate between those generated images and real images present in the training set. A trained GAN is then able to generate realistic images similar to those in the training set. 
%Recently, GANs have been adapted to the task of semi-supervised learning, most commonly by extending the discriminator to determine the specific class of the image in addition to determining whether the image is real or generated \cite{Improved}. While other semi-supervised deep learning methods have been proposed \cite{vat}, GAN-based semi-supervised methods have achieved state-of-the-art results on benchmark natural image datasets \cite{badgan}.
% While the SSL-GANs would learn from the unlabeled data in addition to the labeled subset, they do have the added burden of performing two classification tasks (real vs. fake, and normal vs. abnormal).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%suggests that the labeling burden can be reduced significantly without compromising classification performance. 
%remove VGG and Pretrained
%Later: Image level SSL for small labelled set
%Comment on dependence on resolution
%Cite for best case IDRID challenge dataset performance and compare against leaderboard/publications qualitatively, while noting limitations to compare

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We demonstrate the feasibility of semi-supervised deep learning for classification of abnormalities in two retinal imaging applications. Our results showcase the ability to maintain classification accuracy with reduced labeling burden. 
%leverage unlabeled medical images to improve classification performance and enable substantial reductions in the annotation burden.
%for any problem that cannot be pretrained and has problems of overfitting, inter-rater variability, large image sizes, we propose modular learning 
%We anticipate that efforts to enhance semi-supervised deep learning pipelines for higher resolution images and more imbalanced datasets will enhance potential medical imaging applications. 

Discussion Points
%GAN-based semi-supervised deep learning (SSL) approaches have shown potential in computer vision tasks, but have limited application to the high-resolution images seen in many medical applications. 

%in an interpretable manner
%gross features covering large extent of image vs. specks, resolution requirements

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Kaggle Dataset}: We validated the models trained on the IDRiD dataset for adaptation on color retinal fundus photographs from the independent Kaggle Diabetic Retinopathy cohort and dataset. Specifically, we employed the public images in the Kaggle test set comprising 10,000 fundus photographs from multiple primary care sites with severity ratings from licensed clinicians. We posed a binary classification task that is most similar to the IDRiD task – namely to distinguish healthy (Kaggle severity scale of 0) vs. referable disease (Kaggle severity scale of 2-4). 
%For each retinal image, severity was rated  on a scale of 0 (healthy), 1 (mild), 2 (moderate), 3 (severe), and 4 (proliferative). We posed the classification problem as a binary task, and dichotomized labels as `healthy' (scale of 0) or `diseased' (scale of 2-4), and excluded mild diabetic retinopathy images (scale 1). 
% We randomly sampled 12,000 images from the full dataset for our experiments, used only left-eye images (to avoid left-right correlations), and corrected for the variability in camera models, focus, exposures, and resolutions in the raw images by (a) rescaling the images to a radius of 300, (b) local color averaging, (c) image clipping, and (d) normalizing intensity values within each channel across all patients to have mean 0 and standard deviation 1.

% \subsubsection{Validation on an Independent Cohort and Dataset}
% To assess generalizability, we trained semi-supervised and supervised models on the IDRiD dataset and validated on the Kaggle dataset. We used the same pre-processing and data augmentation procedures for both datasets. We report the classification AUC on the Kaggle dataset, and compare performance of the semi-supervised GAN (from 2.4.1) against the baseline pretrained ResNet50  - both trained on the IDRiD set and applied blind to the Kaggle Test Set. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We show also the performance of a ResNet applied directly at the image-level, and see that \emph<not much difference/loss> in comparison to the ResNet applied for patch-level with voting to combine results for image-level classification. %Comment on dataset imbalanced - by how much
%variability of SSL-GAN vs. CNN
%With decreasing numbers of labeled samples, the performance of the semi-supervised classifier is more robust than that of the supervised baseline. %Later: Regression vs. voting

